A Multi-dimensional Evaluation of Tokenizer-free Multilingual Pretrained Models

Recent work on tokenizer-free multilingual pretrained models show promising results in improving cross-lingual transfer and reducing engineering overhead (Clark et al., 2022; Xue et al., 2022). However, these works mainly focus on reporting accuracy on a limited set of tasks and data settings, placing less emphasis on other important factors when tuning and deploying the models in practice, such as memory usage, inference speed, and fine-tuning data robustness. We attempt to fill this gap by performing a comprehensive empirical comparison of multilingual tokenizer-free and subword-based models considering these various dimensions. Surprisingly, we find that subword-based models might still be the most practical choice in many settings, achieving better performance for lower inference latency and memory usage. Based on these results, we encourage future work in tokenizer-free methods to consider these factors when designing and evaluating new models.

==> fig_inference.tex <==
\begin{figure*}[ht]
\begin{subfigure}{\textwidth}
  \centering
    \includegraphics[width=\textwidth]{figures/memory_efficiency.pdf}
\end{subfigure}\vspace{0em}\\
\begin{subfigure}{\textwidth}
  \centering
    \includegraphics[width=\textwidth]{figures/inference_efficiency.pdf}
\end{subfigure}

\caption{Average XNLI, NER, TyDi QA performance across languages when each model is fine-tuned with multilingual data (mBERT: \textcolor{mbert_color}{\filledsquare{}}, CANINE-S: \textcolor{canine_color}{\filledsquare{}}, mT5: \textcolor{mt5_color}{\filledsquare{}}, ByT5: \textcolor{byt5_color}{\filledsquare{}}), single-language data (mBERT: \textcolor{mbert_color}{\filledcircle{}}, CANINE-S: \textcolor{canine_color}{\filledcircle{}}, mT5: \textcolor{mt5_color}{\filledcircle{}}, ByT5: \textcolor{byt5_color}{\filledcircle{}}), or zero-shot transferred from English (mBERT: \textcolor{mbert_color}{\filledtriangle{}}, CANINE-S: \textcolor{canine_color}{\filledtriangle{}}, mT5: \textcolor{mt5_color}{\filledtriangle{}}, ByT5: \textcolor{byt5_color}{\filledtriangle{}}). The x-axis indicates the corresponding inference cost criteria (Top row: Peak GPU memory, Bottom row: Inference latency) in each task. We additionally use \textcolor{green}{\ding{77}} to mark the direction of the ideal cost and performance.\label{fig:main_result} 
% \xw{for figure 1, make the square/rectangle/start shape in the caption the corresponding color in the plot.
% Make the star bigger in the plot
% }
}
\end{figure*}

==> tab_main_results.tex <==
\begin{table*}[width=\textwidth]
    \centering
    \begin{tabular}{l|ccc|ccc|ccc}
    \toprule
      \multirow{2}{*}{Model}  & \multicolumn{3}{c|}{\textsc{XNLI}} & \multicolumn{3}{c|}{\textsc{NER}} & \multicolumn{3}{c}{\textsc{TyDi QA}} \\
        %  \hline
        & Zeroshot & Single & Multi & Zeroshot & Single & Multi & Zeroshot & Single & Multi \\
        \hline
      mBERT   & 65.4 & 73.1 & 74.7 & 58.2 & 88.5 & 88.4 & 56.51 & 75.17 & 78.39 \\
        \hline
      CANINE-S   & 53.8 & 68.6 & 69.4 & 43.4 & 82.7 & 86.1 & 34.91 & 67.65 & 74.13 \\
      CANINE-C   & 55.0 & 66.8 & 69.0 & 45.8 & 82.0 & 85.9 & 31.39 & 65.56 & 74.55 \\
        \hline
       mT5 & 63.0 & 69.5 & 72.7 & 47.2 & 80.1 & 79.9 & 38.54 & 68.09 & 72.05\\
        % \hline
       ByT5 & 67.2 & 73.0 & 74.7 & 46.9 & 80.7 & 82.4 & 43.09 & 72.97 & 74.48\\
    \bottomrule
    \end{tabular}
    \caption{Average performance across languages for different tasks and models.}
    \label{tab:main_results}
\end{table*}
